Polling Latent Opinions: A Method for Computational Sociolinguistics Using Transformer Language Models

Text analysis of social media for sentiment, topic analysis, and other analysis depends initially on the selection of keywords and phrases that will be used to create the research corpora. However, keywords that researchers choose may occur infrequently, leading to errors that arise from using small samples. In this paper, we use the capacity for memorization, interpolation, and extrapolation of Transformer Language Models such as the GPT series to learn the linguistic behaviors of a subgroup within larger corpora of Yelp reviews. We then use prompt-based queries to generate synthetic text that can be analyzed to produce insights into specific opinions held by the populations that the models were trained on. Once learned, more specific sentiment queries can be made of the model with high levels of accuracy when compared to traditional keyword searches. We show that even in cases where a specific keyphrase is limited or not present at all in the training corpora, the GPT is able to accurately generate large volumes of text that have the correct sentiment.

==> text/acknowledgements.tex <==
\section*{Acknowledgements}

Thanks to everyone who helped! In particular, we would like to thank...

==> text/appendices.tex <==
\appendix

\section{Example Appendix}
\label{sec:appendix}

This is an appendix.

==> text/floober.tex <==
\subsection{The Floober}
Contextual interpoation examples by the GPT-3

\textbf{The Floober is a large flightless bird that lives in semi-arid areas in Africa. Like its cousin the Ostrich}, it is capable of running at speeds of up to 60 miles per hour. It uses its long legs and claws to dig in the sand and expose roots and tubers. The Floober also has a sharp beak that can crack and peel bark from trees, allowing the bird to eat the inner bark.  The Floober has a keen sense of smell, much like a pig. In fact, it was first located when it was discovered that it was destroying the crops of local farmers by uprooting them. Unfortunately for the farmers, once they had located the Floober, they could not find a way to eliminate the bird without damaging the local ecosystem. It was later discovered that the Floober eats a specialized type of fungus that is prevalent in its habitat, and the farmers eventually learned to live with their new neighbor.

\textbf{The Floober is a large flightless bird that lives in semi-arid areas in Africa. Like its cousin the Ostrich}, the Floober is a member of the Struthionidae family.  The Floober was discovered in the early 19th century by explorers and naturalists like William Cornwallis Harris, who named them after the sound they made: "Floober". They were first described in 1821 by Thomas Burchell, the discoverer of Burchell's zebra. Other species were later discovered, including the Giant Floober and the Calico Floober. The Giant Floober is known only from fossils and was probably hunted to extinction by humans. Modern science recognizes two species of Floobers, the Eastern Floober, which is found in the savannas and grasslands of central Africa, and the Western Floober, which is found in the savannas and grasslands of southern Africa.

==> text/useful_links.tex <==
\appendix

\section{Useful Links}
\begin{itemize}
    \item Conference Home: \url{https://2022.naacl.org/}
    \item Call for papers: \url{https://2022.naacl.org/calls/papers/}
    \item Author policies: \url{https://aclrollingreview.org/cfp#authorship}
    \item Word embeddings quantify 100 years of gender and ethnic stereotypes: \url{https://www.pnas.org/content/pnas/115/16/E3635.full.pdf}
    \item Dynamic Word Embeddings for Evolving Semantic Discovery: \url{https://arxiv.org/abs/1703.00607}
    \item Inferring Mechanisms for Global Constitutional Progress: \url{https://arxiv.org/abs/1606.04012}
    \item Mark Pagel Professor of Evolutionary Biology \url{https://scholar.google.com/citations?hl=en&user=ddDQGCYAAAAJ}
    \item Claire Bowern Professor of Linguistics, Yale University \url{https://scholar.google.com/citations?hl=en&user=uLun3nEAAAAJ}
    \item Russell D. Gray Max Planck Institute for Evolutionary Anthropology \url{https://scholar.google.com/citations?hl=en&user=sksPd1cAAAAJ}
\end{itemize}
